Scalable Betweenness Centrality Maximization via Sampling

Betweenness centrality is a fundamental centrality measure in social network analysis. Given a large-scale network, how can we find the most central nodes? This question is of key importance to numerous important applications that rely on betweenness centrality, including community detection and understanding graph vulnerability. Despite the large amount of work on designing scalable approximation algorithms for betweenness centrality, estimating it on large-scale networks remains a computational challenge. In this paper, we study the Betweenness Centrality Maximization problem: given a graph $G=(V,E)$ and a positive integer $k$, find a set $S^* \subseteq V$ that maximizes betweenness centrality subject to the cardinality constraint $|S^*| \leq k$. We present an efficient randomized algorithm that provides a $(1-1/e-\epsilon)$-approximation with high probability, where $\epsilon>0$. Our results improve the current state-of-the-art result by Yoshida~\cite{yoshida2014almost}. Furthermore, we provide theoretical evidence for the validity of a crucial assumption in the literature of betweenness centrality estimation, namely that in real-world networks $O(|V|^2)$ shortest paths pass through the top-$k$ central nodes, where $k$ is a constant. On the experimental side, we perform an extensive experimental analysis of our method on real-world networks, demonstrate its accuracy and scalability, and study different properties of central nodes. Finally, we provide three graph mining applications of our method.

==> tex/Setup.tex <==
\spara{Experimental Setup} \label{sec:setup}
In our experiments, we assume the graphs are simple (no self-loop or parallel edge) but the edges can be directed. We used publicly available datasets in our experiments\footnote{\url{http://snap.stanford.edu} and \url{http://konect.uni-koblenz.de/networks/dblp_coauthor}}.
Our algorithm is implemented in {\sc C++}. 



==> tex/TimeEvolvingBW.tex <==
%\subsection{Time evolving networks} \label{sec:time}
\spara{Time evolving networks.} Leskovec {\em et al.} studies empirically  properties of 
time-evolving, real world networks \cite{leskovec2007graph}.  
In this section we investigate how \BW of the most central nodes changes as a function of time. 
\hide{\footnote{Note that our goal here is not to develop a dynamic algorithm with good amortized time per each update of the graph. Instead we seek an algorithm that works very fast on massive static networks, and use for each timestamp separately.}}


We study two temporal datasets, the \textsf{DBLP} \footnote{\babis{what do you mean?}Timestamps are Unix time and can be negative.} and \textsf{Autonomous Systems} (AS) datasets. We also generate stochastic Kronecker graphs on $2^i$ vertices for $i\in\set{8,\ldots,20}$, using $\left(\begin{smallmatrix} 0.9 & 0.5\\ 0.5 & 0.2 \end{smallmatrix}\right)$ as the core-periphery seed matrix. We assume that the $i$-th time snapshot for Kronecker graphs corresponds to $2^{i}$ vertices, for $i=8,\ldots,20$. Note that in these evolving sets, the number of nodes also increases along with new edges. Also, note that the main difference between \textsf{DBLP} and \textsf{Autonomous Systems} is that for \textsf{DBLP} edges and nodes only can be added, where in \textsf{Autonomous Systems} nodes and edges can be increased and decreased.

 
%For each index $i$ we generate \reminder{10 instances} and report averages. 

The results are plotted in logarithmic scale (Fig.~\ref{fig:timeevolving}), and as shown, we observe that the centrality of the highly central set of nodes increases. Also, we observe that the model of stochastic Kronecker graphs behaves similar to the real-world evolving networks with respect to these parameters. 
%does well (i.e., similar to real-world networks) with respect to these parameters, i.e., the core-periphery seed matrix $\left(\begin{smallmatrix} 0.9 & 0.5\\ 0.5 & 0.2 \end{smallmatrix}\right)$.

% stochastic Krone and the Kronecker graphs behave similarly to real-world networks.


% with exponential rate,  and real-world networks’ behavior over time is similar to what stochastic Kronecker graphs models.


%what happens with respect to the most central vertex in the network with respect to \BW as the network changes over time. 



\begin{figure}[t]
\centering
\begin{tabular}{@{}c@{}@{\ }c@{}}
\includegraphics[width=0.49\textwidth]{figures/evolve/AS-1.pdf} &
\includegraphics[width=0.49\textwidth]{figures/evolve/AS-50.pdf} \\
(a) AS: $k=1$ & (b) AS: $k=50$ \\ 
\includegraphics[width=0.49\textwidth]{figures/evolve/db-1.pdf} &
\includegraphics[width=0.49\textwidth]{figures/evolve/db-50.pdf} \\
(a) DBLP: $k=1$ & (b) DBLP: $k=50$ \\ 
\includegraphics[width=0.49\textwidth]{figures/evolve/KG-1.pdf} &
\includegraphics[width=0.49\textwidth]{figures/evolve/KG-50.pdf} \\
(a) KG: $k=1$ & (b) KG:  $k=50$
\end{tabular}
\caption{\label{fig:timeevolving} \small Largest betweenness centrality score 
and number of nodes, edges and average degree versus time on the (i) 
\textsf{Autonomous systems}  (a),(b) (ii) \textsf{DBLP} dataset  (c),(d)
and (iii) stochastic Kronecker graphs (e),(f).}
\vspace{-4mm}
\end{figure}






==> tex/macro.tex <==
\usepackage{amsmath}
%\usepackage{unicode-math}
\usepackage{amsfonts}
%\usepackage{algorithm,algorithmic}
%\usepackage{amssymb,bbm}
\usepackage{latexsym}
\usepackage{graphicx}
\usepackage{color}
\usepackage{url}
\usepackage{xspace} 
%\usepackage[algoruled,vlined]{algorithm2e}
\usepackage{algpseudocode}
\usepackage{authblk}
\usepackage{soul}
%\usepackage[show]{notes-alt}

\usepackage{floatrow}

\usepackage[sc]{mathpazo}
\usepackage{multirow}
\usepackage{adjustbox}
\usepackage{booktabs}
\usepackage{caption}
\usepackage{subcaption}


%\floatname{algorithm}{Procedure}
%\renewcommand{\algorithmicrequire}{\textbf{Input:}}
%\renewcommand{\algorithmicensure}{\textbf{Output:}


\definecolor{ForestGreen}{rgb}{0.1333,0.5451,0.1333}
\usepackage[letterpaper,
            colorlinks,linkcolor=ForestGreen,citecolor=ForestGreen,
            backref,
            bookmarks,bookmarksopen,bookmarksnumbered]{hyperref}


\newcommand{\field}[1]{\mathbb{#1}} % requires 
%\newtheorem{theorem}{Theorem}
%
%\newtheorem{lemma}{Lemma}
%\newtheorem{proposition}{Proposition}
%\newtheorem{definition}{Definition}
%\newcommand{\spara}[1]{\smallskip\noindent{\bf #1}\ }
%\newcommand{\mpara}[1]{\medskip\noindent{\bf #1}\ }
%\newcommand{\para}[1]{\noindent{\bf #1}\ }
\newcommand{\hide}[1]{}
 
%% tight spacing in item lists
\newcommand{\squishlist}{
 \begin{list}{$\bullet$}
  {  \setlength{\itemsep}{0pt}
     \setlength{\parsep}{3pt}
     \setlength{\topsep}{3pt}
     \setlength{\partopsep}{0pt}
     \setlength{\leftmargin}{2em}
     \setlength{\labelwidth}{1.5em}
     \setlength{\labelsep}{0.5em}
} }
\newcommand{\squishlisttight}{
 \begin{list}{$\bullet$}
  { \setlength{\itemsep}{0pt}
    \setlength{\parsep}{0pt}
    \setlength{\topsep}{0pt}
    \setlength{\partopsep}{0pt}
    \setlength{\leftmargin}{2em}
    \setlength{\labelwidth}{1.5em}
    \setlength{\labelsep}{0.5em}
} }

\newcommand{\squishdesc}{
 \begin{list}{}
  {  \setlength{\itemsep}{0pt}
     \setlength{\parsep}{3pt}
     \setlength{\topsep}{3pt}
     \setlength{\partopsep}{0pt}
     \setlength{\leftmargin}{1em}
     \setlength{\labelwidth}{1.5em}
     \setlength{\labelsep}{0.5em}
} }

\newcommand{\squishend}{
  \end{list}
}

\newcommand{\squishlistt}{
 \begin{list}{---}
  {  \setlength{\itemsep}{0pt}
     \setlength{\parsep}{3pt}
     \setlength{\topsep}{3pt}
     \setlength{\partopsep}{0pt}
     \setlength{\leftmargin}{2em}
     \setlength{\labelwidth}{1.5em}
     \setlength{\labelsep}{0.5em}
} }
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\newcommand{\blue}[1]{{\it\bf \color{magenta}#1}}
\newcommand{\reminder}[1]{{\it\bf \color{red}**#1**}}
\newcommand{\obs}[1]{{\it\bf Observation: \color{blue} #1}}
\newcommand{\Prob}[1]{\ensuremath{{\bf{Pr}}\left[{#1}\right]}}
\newcommand{\Mean}[1]{\ensuremath{{\mathbb E}\left[{#1}\right]}}
\newcommand{\NP}{\ensuremath{\mathbf{NP}}\xspace}
\newcommand{\NPhard}{{\ensuremath{\mathbf{NP}}-hard}\xspace}
\newcommand{\NPcomplete}{{\ensuremath{\mathbf{NP}}-complete}\xspace}
\newcommand{\sgn}{{\ensuremath{\mathrm{sgn}}}}
\newcommand{\whp}{\textit{whp}\xspace}
\newcommand{\Var}[1]{{\mathbb Var}\left[{#1}\right]}
\newcommand{\mixing}{t_{\text{mix}}(\epsilon)}
%\newtheorem{corollary}{Corollary}
%  \newtheorem{definition}{Definition}
\newtheorem{remark}{Remark}
\newcommand{\ahmad}[1]{\textcolor{red}{#1}}
\newcommand{\babis}[1]{\textcolor{blue}{(#1)}}

\DeclareMathOperator*{\argmax}{arg\,max}

\newcommand{\paran}[1]{\left(#1\right)}
\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\setof}[2]{\left\{#1 \vert #2\right\}}
\newcommand{\E}[1]{\mathbb{E}\left(#1\right)}
\newcommand{\pr}[1]{\text{Pr}\left(#1\right)}
% \newcommand{\cost}[1]{\texttt{cost}\left(#1\right)}



\def\cost{\texttt{cost}}
% \def\adsch{\texttt{adopting\_schedule}}
% \def\C{\texttt{compute\_c}}
\def\R{\mathcal{R}}
\def\A{\mathcal{A}}
% \def\H{\mathcal{S}}
\def\H{\mathcal{H}}
\def\inf{\texttt{inf}}
\def\opt{\texttt{MAX}}
\def\cond{\texttt{cond}}

\def\approx{\texttt{APPROX}}
\def\topk{\texttt{TopK}}
\def\peel{\texttt{Peel}}
\def\infmax{\texttt{INFMAX}}

\def\he{hyper-edge}
\def\He{Hyper-edge} 


\newcommand{\CMP}{ \textsc{CMP}\xspace}

\newcommand*{\algonamebase}{HEDGE}
\newcommand*{\algonamebasecaps}{HEDGE}
\newcommand*{\algonamebasecap}{Hedge}
\newcommand*{\algoname}{\texttt{\algonamebase}\xspace}

\newcommand*{\exnamebase}{EXHAUST}
\newcommand*{\exnamebasecaps}{EXHAUST}
\newcommand*{\exnamebasecap}{Exhaust}
\newcommand*{\exname}{\texttt{\exnamebase}\xspace}












